Logic Blog 2017

The blog is somewhat shorter than in previous years, It contains new insights in a variety of areas, including computability, quantum algorithmic version of the SMB theorem, descriptions of groups (both discrete and profinite), metric spaces. There are also lots of open questions in computability, randomness, and computable model theory.

==> sections2017/Nies_Tent_May.tex <==
\section{Nies and Tent:  mutual, and bi-interpretability of $\omega$-categorical structures}

   

%Hi everyone. 
Recall that to interpret a structure $A$ in a structure $B$, one needs a $\emptyset$-definable set $D$ of $d$-tuples in $B$, and a definable equivalence relation on $D$. The elements of $A$ are represented by elements of $D/E$.   The number $d$ is called the dimension of the interpretation. One often writes $A = \Gamma(B)$, where $\Gamma$ is the decoding function given by a scheme of formulas; besides $D$ and $E$, for each symbol in the language  of $A$ one has a corresponding formula.
For background on interpretations and bi-interpretability  see Hodges \cite[Ch.\ 5]{Hodges:93}. 

 Nies, Schlicht and  Tent work on the   complexity of  the eqivalence relation of  bi-interpre\-tability for  $\omega$-categorical  structures.  By Ahlbrandt and Ziegler, two such structures are bi-interpretable iff there automorphism groups are topologically isomorphic.  
 
 Given that countable structures form a Polish space, the appropriate framework is Borel reducibility.   The equivalence relation is Borel (Nies, Schlicht and Tent), and below graph isomorphism (Kechris, Nies and Tent). The only known lower bound is at present the identity on $\mathbb R$. 
 
 
 
 \subsection{Mutual interpretability is above $E_0$}  If we  replace  bi-interpretability by the weaker mutual interpre\-tability (which merely says that each structure can be interpreted in the other), we can show non-smoothness, but also may lose the   upper bound of graph isomorphism. Note that mutual interpretability is strictly weaker; consider  e.g.\ an infinite set, and an equivalence relation on a countable domain with all classes of size $2$. 
 
 Recall that $E_0$ is the Borel equivalence relation of eventual equality among infinite bit sequences, or equivalently, of  subsets of $\omega$. 

\begin{thm} \mbox{} 

$E_0$ is Borel reducible to mutual interpretability of $\omega$-categorical structures. \end{thm}



For each $k$ we have a $k$-ary relation symbol $R_k$. Let $G_{\{k\}}$ be the random $k$-hypergraph (irreflexive, symmetric). More generally,  for $W \sub \NN$ let  $\+ C_W$ be  the class of all finite structures $M$ in the language $L(\{R_k \colon k \in W\})$ such that $R_k^M$ is a set of  $k$-hyperedges for $k \in W$. Clearly $\+ C_W$ has the usual properties HP, JEP and AP.  Let $G_W$ be the Fraisse limit of $\+ C_W$.   Note that the theory of $G_W$ has quantifier elimination (QE) because the language is relational.


\begin{lemma} \label{lem: interpret} For $k\ge 2$, the structure $G_{\{k\}} $ cannot be interpreted in $G_{\{1, \ldots, k-1\}}$. \end{lemma}
\begin{proof}  This is clearly true for $k=2$, so we may suppose that  $k \ge 3$.  Assume for a contradiction  there is such an interpretation $\Gamma$, of dimension $d$.
By QE, each $k$-hypergraph of size $n$ is interpreted via $\Gamma$ in a $\+ C_W$-structure of size at most $dn$. Write $C(u,w)= \binom u w$. There are at least $\tp{C(n,k)}/ n!$ non-isomorphic $k$--hypergraphs of size $n$. On the other hand,  there are at most $\prod_{i<k} \tp{C(dn,i)}$  many $L(\{R_i\colon i< k\})$ structures of size $dn$. So for each $n$ we have 

$$\tp{C(n,k)}/ n! \le \prod_{i<k} \tp{C(dn,i)}.$$
Taking the   logarithm  in base 2 yields   $C(n,k) - \sum_{i \le n} \log i \le \sum_{i < k} C(dn,i)$. This clearly fails for large enough $n$ because $\sum_{i \le n} \log i \le n^2$, and the polynomial $C(n,k)- n^2$ has degree greater than the polynomial $\sum_{i < k} C(dn,i)$. \end{proof}


\begin{proof}[Proof of the Theorem] We say that a set  $X \sub \omega$ is \emph{nice} if it contains the odd numbers, $0 \not \in X$,  and $2n(n+1) \in X$ implies $2n(n+1) + 2i \in X$ for each  $i < n$. Clearly $E_0$  is Borel equivalent to $E_0$ restricted to nice sets. So it suffices to reduce this  restricted  equivalence relation to mutual interpretability of $\omega$-categorical structures.  

Let $M_X= G_{\{ 2^r \colon r \in X\}}$. 
\begin{claim} For nice sets $X , Y$ we have 

$X - Y $ finite $\LR$ $M_X $ can be interpreted in $M_Y$. 
\end{claim}

\n 
$\RA$: Let  $v$ be the least even number such that $m \in X, m \ge v$ implies $m \in Y$. We define an interpretation $\Gamma$ of $M_X$ in $M_Y$ of dimension $2^v$. The domain $D$ is the set of $2^v$-tuples of pairwise distinct elements  $z_1, \ldots, z_{2^v}$ such that $i< j \lra R_2 z_i z_j$.    (We could also use the ordered random hypergraphs here. For that we would replace $R_2$ by a dense linear order without end points.)
 The equivalence relation $E$  is identity. 
The relation symbol $R_{2^i}$ for $i\in X$ is interpreted by a formula $\phi_i (y_1, \ldots, y_{2^i})$ defined next, where each $y_r$ is a $2^v$-tuple.   

The formula $\phi_i$ firstly expresses that the tuples are in $D$, and  are disjoint when viewed as sets. Secondly, if  $i$ is  even and  $i < v$, the formula   expresses that  $R_{2^{i+1}}$ holds for $  \hat y_1, \ldots, \hat y_{2^i}$, where $\hat y_i $ consists of the first two elements of the tuple w.r.t.\ the linear order given by $R_2$; otherwise,   $\phi_i$ expresses that    $R_{2^{i+v}}$ holds for $\phi_i (y_1, \ldots, y_{2^i})$.

Note that the formula to interpret a relation $R^X_{2^i}$    uses $R_2$ and  $R^Y_{2^{i+1}}$ for $i < v$ in the first case, and    $R^Y_{2^{i+v}}$ otherwise. So no relation of $Y$ other than $R_2$  is used twice. This easily   implies that $\Gamma(M_Y)$ is the random structure for the language of $M_X$, and hence isomorphic to  $M_X$. 





\n 
$\LA$: Suppose there is   an interpretation $\Gamma$, of dimension  $q$, such that $M_X = \Gamma(M_Y)$.  Assume for a contradiction there is $n >  \log q$ such that $\ell= 2n(n+1) \in X -Y$. Let $\phi(  y_1, \ldots, y_{2^\ell})$ be the formula for $R_{2^\ell}$. Since   $2n(n+1)+2i \not \in Y$ for $i< n$, and the theory of $M_Y$ has QE, $\phi$ can only contain relation symbols $R_{2^v}$ for $v< \ell$.   This contradicts Lemma~\ref{lem: interpret} with $k = \tp \ell$.
\end{proof}



\subsection{Bi-interpretability is smooth for the very restricted case without equivalence relations}

Let $S$ be a finite relational language. Upon an effective numbering of $L(S)$, the space of complete theories $T$  in $L(S)$ can be seen as a closed subset of Cantor space $\cantor$. To have QE is also closed: the language is finite, so there are only finitely possibilities for a quantifier free formulae equivalent to a fmla $\ex x \psi(\ol y, x)$ where $\psi $ is quantifier free. The QE theories correspond to Fraisse limits, as they are $\omega$ categorical (only finitely many $n$-types for each $n$) and homogeneous.  

Let us say two theories $S,T$ are strongly bi-interpretable 
















